The Elasticity of Quantitative Investment

What is the demand elasticity of statistical arbitrageurs that invest according to the advice of modern cross-sectional asset pricing models? Thirteen models from the literature exhibit strikingly inelastic demand, in contrast to classical models that rely on statistical arbitrageurs to create elastic market demand for assets. This inelasticity arises from the difficulty of trading against price changes. A quantitative equilibrium model shows that aggregate demand remains inelastic even with these statistical arbitrageurs in the market.

==> figures/four_categories.tex <==
\begin{tikzpicture}
\draw[red, very thick] (-4,0) rectangle (1,1);
\draw[red, very thick] (-4,-2) rectangle (1,-1);
\draw[blue, very thick] (-4,-0.5) rectangle (1,0);
\draw[blue, very thick] (-4,-1) rectangle (1,-0.5);
%\draw[orange, ultra thick] (4,0) -- (6,0) -- (5.7,2) -- cycle;
\draw[<->,thick] (-4.2,-2) --  (-4.2,1);
\node[text width=3cm] at (-3.1,-0.5) {$\alpha$};
\draw[<-,thick] (1.05, -0.5) -- (1.5, -0.5) node [right] {$\alpha = 0$};
\draw[<-,thick] (1.05, 0) -- (1.5, 0) node [right] {$\alpha = \bar \alpha$};
\draw[<-,thick] (1.05, -1) -- (1.5, -1) node [right] {$\alpha = -\bar \alpha$};
\draw[<-,thick] (1.05, 0.5) -- (1.5, 0.5) node [right] {$\alpha > \bar \alpha$};
\draw[<-,thick] (1.05, -1.5) -- (1.5, -1.5) node [right] {$\alpha < -\bar \alpha$};
\node[text centered] at (-1.5,0.5) {Amplification};
\node[text centered] at (-1.5,-1.5) {Severe Overcorrection};
\node[text centered] at (-1.5,-0.25) {Correction};
\node[text centered] at (-1.5,-0.75) {Overcorrection};
\draw[<->,thick] (3.2,1) -- (3.2,-2);
\draw[-,thick] (3.1,0) -- (3.3,0);
\draw[red,->,thick] (-1.5,1) -- (-1.5,1.3);
\draw[red,->,thick] (-1.5,-2) -- (-1.5,-2.3);
\end{tikzpicture}

==> tables/demand_elasticity.tex <==
\begin{tabular}{@{\extracolsep{4pt}}lllllcccccc}
% \\[-1.8ex]\hline
% \hline \\[-1.8ex]
\toprule
 & & & & & $\eta_{i,t}$ & $\frac{\beta_{i,1,t} P_{i,t}}{w_{i,t} A_t}$ & $\frac{\beta_{i,2,t}}{w_{i,t} A_t}$ \\
\\[-1.8ex]
\cline{1-2} \cline{3-5} \cline{6-8} \cline{9-9} \\[-1.8ex]
 & & Level & Log & Additional \\
Row & Model & Covariate & Covariate & Covariates ($\dot z_{i,k,t}$) & Elasticity & Level term & Log term & $R^2$ \\
\hline \\[-1.8ex]

1 & KY & Yes (KY) & None & EKY & 0.550$^{***}$ & 0.450$^{***}$ & & 10.9 \\
 & & & & & (0.014) & (0.014) \\
\\[-1.8ex]


2 & Generalized & Yes & None & None & 0.348$^{***}$ & 0.652$^{***}$ & & 7.8 \\
& & & & & (0.002) & (0.002) &\\
\\[-1.8ex]

3 & Generalized & Yes & None & EKY & 0.675$^{***}$ & 0.325$^{***}$ & & 26.5 \\
& & & & & (0.005) & (0.005) & \\
\\[-1.8ex]

4 & Generalized & Yes & Yes & KY & 5.153$^{***}$ & 0.323$^{***}$ & -4.476$^{***}$ & 26.7 \\
& & & & & (0.209) & (0.005) & (0.208) \\
\\[-1.8ex]

5 & Generalized & Yes & Yes & KY \& Exog & 9.937$^{***}$ & 0.608$^{***}$ & -9.545$^{***}$ & 35.7 \\
& & & & & (0.416) & (0.002) & (0.415) \\
\\[-1.8ex]

6 & Generalized & Yes & Yes & All & 11.667$^{***}$ & 0.571$^{***}$ & -11.238$^{***}$ & 38.2 \\
& & & & & (0.501) & (0.003) & (0.501) \\
\\[-1.8ex]

\hline \\[-1.8ex]
\multicolumn{2}{l}{Observations} & & & & 1,253,175 & 1,253,175 & 1,253,175 \\
% \multicolumn{2}{l}{Months} & & 360 & 360 & 360 \\
% \hline
% \hline \\[-1.8ex]
\bottomrule
\textit{Note:} & & & & \multicolumn{5}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}

==> tables/idio_wealth_effects.tex <==
\begin{tabular}{@{\extracolsep{5pt}}ccccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\multicolumn{13}{c}{\textit{Elasticity Impact from Wealth Effects}} \
\cr \cline{1-13}
\\[-1.8ex] \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex] (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\\[-1.8ex] \hline \\[-1.4ex]

-0.0001 & -0.0007 & -0.0021 & -0.0011 & -0.0006 & -0.0007 & -0.0011 & -0.0012 & -0.001 & -0.0011 & 0.0000 & -0.0015 & -0.0001 \\
\hline
\hline \\[-1.8ex]
\end{tabular}

==> tables/lf_regs.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lcccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{12}{c}{\textit{Dependent Variable: Log Mispricing}} \
\cr \cline{2-13}
\\[-1.8ex] & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\

\hline \\[-1.8ex]
 $\theta_t$ & -0.286$^{}$ & 0.197$^{}$ & 0.212$^{*}$ & -0.312$^{***}$ & -0.315$^{***}$ & -0.358$^{***}$ & -0.079$^{***}$ & -0.183$^{***}$ & 1.444$^{***}$ & 0.093$^{}$ & 16.534$^{***}$ & 0.092$^{}$ \\
& (0.763) & (0.157) & (0.111) & (0.064) & (0.033) & (0.058) & (0.014) & (0.025) & (0.106) & (0.145) & (5.599) & (0.074) \\
\hline \\[-1.8ex]
Month FE & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes & Yes \\
 Obs. & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 & 2880 \\
 $R^2$ & 0.002 & 0.031 & 0.025 & 0.168 & 0.641 & 0.286 & 0.340 & 0.439 & 0.537 & 0.013 & 0.002 & 0.051 \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{12}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}

==> tables/lf_table_log.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccccccc}

\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] 
& \multicolumn{13}{c}{Average Learning Fraction $(\theta_t)$, February 2010 - January 2020} \\ \cline{2-14}
\\[-1.8ex] 
\\[-1.8ex] IAF $\theta_0$ & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex]
\hline \\[-1.8ex]


0.0001 &   0.0006 & 0.0009 & 0.001 & 0.0001 & 0.0058 & 0.0087 & 0.0096 & 0.0001 & 0.0634 & 0.0013 & 0.0001 & 0.0002 & 0.0004 \\
\\[-1.8ex]
0.0005 &   0.0001 & 0.0015 & 0.001 & 0.0001 & 0.0122 & 0.031 & 0.0234 & 0.0001 & 0.0086 & 0.0014 & 0.0005 & 0.0002 & 0.0015 \\
\\[-1.8ex]
0.001 &   0.0001 & 0.0014 & 0.0009 & 0.0001 & 0.0163 & 0.0524 & 0.036 & 0.0001 & 0.0105 & 0.0013 & 0.001 & 0.0002 & 0.0028 \\
\\[-1.8ex]
0.005 &   0.0001 & 0.0022 & 0.0007 & 0.0001 & 0.0269 & 0.1119 & 0.0616 & 0.0001 & 0.0114 & 0.0011 & 0.0045 & 0.0003 & 0.0053 \\
\\[-1.8ex]
0.01 &   0.0001 & 0.0022 & 0.0006 & 0.0001 & 0.0355 & 0.1487 & 0.062 & 0.0001 & 0.0946 & 0.001 & 0.0078 & 0.0001 & 0.01 \\
\\[-1.8ex]
0.05 &   0.0001 & 0.0034 & 0.0006 & 0.0001 & 0.0588 & 0.264 & 0.027 & 0.0001 & 0.0007 & 0.0011 & 0.0098 & 0.0001 & 0.0304 \\
\\[-1.8ex]
0.1 &   0.0001 & 0.0041 & 0.0006 & 0.0001 & 0.0748 & 0.3358 & 0.026 & 0.0001 & 0.0007 & 0.0012 & 0.0026 & 0.0001 & 0.0521 \\
\\[-1.8ex]
0.25 &   0.0001 & 0.0031 & 0.0006 & 0.0001 & 0.0941 & 0.4601 & 0.0875 & 0.0001 & 0.0007 & 0.0014 & 0.0001 & 0.0001 & 0.0001 \\
\\[-1.8ex]



\hline
\hline 
 & \multicolumn{13}{r}{\textit{Note:} $^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\

\end{tabular}


==> tables/mkt_elasticity_robust.tex <==
\begin{tabular}{@{\extracolsep{5pt}}llccccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
 & & \multicolumn{13}{c}{\textit{Change in Aggregate 
 Counterfactual Elasticity for Individual Stocks with Different Statistical Arbitrageurs}} \
\cr \cline{3-15}
\\[-1.8ex] Type & AF $\theta_t$ & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex] & & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline \\[-1.8ex]

Recursive & 0.0 &   0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 & 0.0001 &   0.000 & 0.001 & 0.002 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 \\
 & 0.0005 &   0.000 & 0.001 & 0.001 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 & 0.001 &   0.000 & 0.001 & 0.001 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 & 0.005 &   0.000 & 0.001 & 0.001 & 0.000 & 0.003 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 & 0.01 &   0.000 & 0.001 & 0.001 & 0.000 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 & 0.05 &   0.000 & 0.003 & 0.003 & 0.000 & 0.006 & 0.000 & 0.000 & 0.006 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 \\
 & 0.1 &   0.000 & 0.005 & 0.004 & 0.000 & 0.003 & 0.000 & 0.001 & 0.004 & 0.000 & 0.004 & 0.000 & 0.000 & 0.000 \\
 & 0.25 &   0.000 & 0.01 & 0.009 & 0.000 & 0.000 & 0.000 & 0.001 & 0.004 & 0.000 & 0.011 & 0.000 & 0.000 & 0.000 \\

\hline \\[-1.8ex]

Double Elas. & 0.0 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
 & 0.0001 &   0.000 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
 & 0.0005 &   0.000 & 0.004 & 0.006 & 0.000 & 0.002 & 0.001 & 0.001 & 0.000 & 0.000 & 0.006 & 0.000 & 0.000 & 0.000 \\
 & 0.001 &   0.000 & 0.005 & 0.005 & 0.000 & 0.003 & 0.002 & 0.002 & 0.000 & 0.000 & 0.011 & 0.000 & 0.000 & 0.000 \\
 & 0.005 &   -0.001 & 0.001 & 0.014 & -0.001 & 0.009 & 0.001 & -0.003 & 0.000 & -0.003 & -0.003 & -0.001 & -0.001 & -0.001 \\
 & 0.01 &   -0.003 & 0.002 & 0.027 & -0.003 & 0.011 & -0.003 & -0.006 & 0.000 & -0.007 & -0.006 & -0.002 & -0.003 & -0.003 \\
 & 0.05 &   -0.013 & 0.003 & 0.019 & -0.013 & 0.007 & -0.036 & -0.03 & -0.003 & -0.033 & -0.029 & -0.013 & -0.013 & -0.013 \\
 & 0.1 &   -0.027 & 0.016 & 0.001 & -0.026 & -0.002 & -0.073 & -0.059 & -0.014 & -0.069 & -0.057 & -0.026 & -0.026 & -0.027 \\
 & 0.25 &   -0.067 & 0.018 & -0.047 & -0.067 & -0.035 & -0.174 & -0.148 & -0.033 & -0.17 & -0.138 & -0.066 & -0.067 & -0.067 \\

\hline
\hline \\[-1.8ex]
\end{tabular}


==> tables/mkt_elasticity_simple_5win.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
 & \multicolumn{13}{c}{\textit{Change in Aggregate 
 Counterfactual Elasticity for Individual Stocks with Different Statistical Arbitrageurs}} \
\cr \cline{2-14}
\\[-1.8ex] AF $\theta_t$ & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline \\[-1.8ex]

0.0001 &   0.000 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
0.0005 &   0.000 & 0.001 & 0.002 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
0.001 &   0.000 & 0.001 & 0.004 & 0.000 & 0.003 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
0.005 &   0.001 & 0.003 & 0.009 & 0.001 & 0.008 & -0.001 & -0.001 & 0.002 & -0.002 & -0.001 & 0.001 & 0.001 & 0.001 \\
0.01 &   0.002 & 0.005 & 0.014 & 0.001 & 0.01 & -0.003 & -0.002 & 0.003 & -0.003 & -0.002 & 0.001 & 0.001 & 0.001 \\
0.05 &   0.007 & 0.028 & 0.03 & 0.007 & 0.02 & -0.014 & -0.01 & 0.017 & -0.014 & -0.008 & 0.007 & 0.007 & 0.007 \\
0.1 &   0.013 & 0.044 & 0.007 & 0.013 & 0.03 & -0.028 & -0.019 & 0.02 & -0.028 & -0.015 & 0.014 & 0.015 & 0.013 \\
0.25 &   0.033 & 0.109 & 0.017 & 0.033 & 0.053 & -0.079 & -0.048 & 0.066 & -0.069 & -0.065 & 0.034 & 0.033 & 0.033 \\



\hline
\hline \\[-1.8ex]
\end{tabular}


==> tables/mkt_elasticity_simple_nowin.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
 & \multicolumn{13}{c}{\textit{Change in Aggregate 
 Counterfactual Elasticity for Individual Stocks with Different Statistical Arbitrageurs}} \
\cr \cline{2-14}
\\[-1.8ex] AF $\theta_t$ & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline \\[-1.8ex]

0.0 &   0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
0.0001 &   0.000 & 0.001 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
0.0005 &   0.000 & 0.001 & 0.002 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
0.001 &   0.000 & 0.001 & 0.004 & 0.000 & 0.004 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
0.005 &   0.001 & 0.003 & 0.009 & 0.001 & 0.009 & -0.003 & -0.002 & 0.003 & -0.003 & -0.002 & 0.001 & 0.001 & 0.001 \\
0.01 &   0.002 & 0.006 & 0.013 & 0.002 & 0.012 & -0.006 & -0.004 & 0.004 & -0.006 & -0.005 & 0.002 & 0.002 & 0.002 \\
0.05 &   0.009 & 0.03 & 0.025 & 0.009 & 0.025 & -0.03 & -0.023 & 0.019 & -0.029 & -0.023 & 0.009 & 0.009 & 0.009 \\
0.1 &   0.018 & 0.05 & -0.004 & 0.018 & 0.037 & -0.06 & -0.044 & 0.025 & -0.059 & -0.042 & 0.019 & 0.02 & 0.018 \\
0.25 &   0.046 & 0.122 & -0.018 & 0.046 & 0.069 & -0.165 & -0.11 & 0.078 & -0.147 & -0.148 & 0.047 & 0.046 & 0.046 \\

\hline
\hline \\[-1.8ex]
\end{tabular}

==> tables/ml_returns_recent10.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline \\[-1.8ex]
 $\alpha$ & -1.789$^{}$ & 21.661$^{***}$ & 17.039$^{***}$ & 5.665$^{}$ & -0.538$^{}$ & 0.555$^{}$ & 12.147$^{***}$ & 34.545$^{***}$ & 0.582$^{}$ & 26.757$^{***}$ & 4.977$^{}$ & 4.135$^{}$ & -0.999$^{}$ \\
& (1.933) & (4.164) & (3.870) & (4.083) & (3.629) & (3.507) & (3.816) & (4.240) & (3.286) & (4.020) & (4.167) & (2.936) & (2.067) \\
 $\beta$ & 0.890$^{***}$ & 0.190$^{**}$ & 0.409$^{***}$ & -0.271$^{***}$ & 0.518$^{***}$ & 0.562$^{***}$ & 0.437$^{***}$ & 0.031$^{}$ & 0.632$^{***}$ & 0.319$^{***}$ & -0.187$^{**}$ & 0.722$^{***}$ & 0.873$^{***}$ \\
& (0.042) & (0.090) & (0.084) & (0.089) & (0.079) & (0.076) & (0.083) & (0.092) & (0.071) & (0.087) & (0.090) & (0.064) & (0.045) \\
\hline \\[-1.8ex]
 Observations & 120 & 120 & 120 & 120 & 120 & 120 & 120 & 120 & 120 & 120 & 120 & 120 & 120 \\
 $R^2$ & 0.792 & 0.036 & 0.168 & 0.074 & 0.268 & 0.316 & 0.191 & 0.001 & 0.400 & 0.102 & 0.035 & 0.521 & 0.763 \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{13}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}

==> tables/ml_returns_recent15.tex <==
\begin{tabular}{@{\extracolsep{5pt}}lccccccccccccc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
\\[-1.8ex] & \multicolumn{1}{c}{BPZ$_F$} & \multicolumn{1}{c}{BPZ$_L$} & \multicolumn{1}{c}{BSV} & \multicolumn{1}{c}{CRW} & \multicolumn{1}{c}{DGU} & \multicolumn{1}{c}{FF3} & \multicolumn{1}{c}{FF6} & \multicolumn{1}{c}{GKX} & \multicolumn{1}{c}{HXZ} & \multicolumn{1}{c}{KNS} & \multicolumn{1}{c}{KPS} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{RF}  \\
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12) & (13) \\
\hline \\[-1.8ex]
 $\alpha$ & 9.236$^{***}$ & 24.462$^{***}$ & 22.077$^{***}$ & 10.062$^{***}$ & 1.924$^{}$ & 1.389$^{}$ & 12.120$^{***}$ & 34.283$^{***}$ & 1.834$^{}$ & 36.098$^{***}$ & -4.360$^{}$ & 8.229$^{***}$ & 3.214$^{*}$ \\
& (2.919) & (3.672) & (3.638) & (3.533) & (3.210) & (2.933) & (3.153) & (3.659) & (2.689) & (3.671) & (3.645) & (2.759) & (1.924) \\
 $\beta$ & 0.615$^{***}$ & -0.124$^{*}$ & 0.183$^{**}$ & -0.298$^{***}$ & 0.497$^{***}$ & 0.610$^{***}$ & 0.524$^{***}$ & -0.150$^{**}$ & 0.687$^{***}$ & 0.127$^{*}$ & 0.173$^{**}$ & 0.667$^{***}$ & 0.854$^{***}$ \\
& (0.059) & (0.074) & (0.074) & (0.072) & (0.065) & (0.059) & (0.064) & (0.074) & (0.054) & (0.074) & (0.074) & (0.056) & (0.039) \\
\hline \\[-1.8ex]
 Observations & 180 & 180 & 180 & 180 & 180 & 180 & 180 & 180 & 180 & 180 & 180 & 180 & 180 \\
 $R^2$ & 0.378 & 0.015 & 0.033 & 0.089 & 0.247 & 0.372 & 0.274 & 0.022 & 0.472 & 0.016 & 0.030 & 0.444 & 0.730 \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{13}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}

